Narrative Structure in Tropes: A Computational Analysis of `Friends'

Tropes are recurring narrative devices in television and film. We carry out a computational analysis of tropes in the sitcom Friends, using human-curated trope annotations from TVTropes, episode transcripts, and IMDb ratings. Because automatic trope detection remains challenging, we treat existing trope annotations as a curated analytical layer and focus on their downstream narrative and semantic functions. We first examine the relationship between episode-level trope frequency and audience reception. We find a statistically significant positive association between trope count and weighted IMDb ratings, although the modest explanatory power suggests that more than trope density alone explains audience evaluation. We then connect trope annotations to dialogue transcripts and represent trope-related dialogue using TF-IDF-based semantic features. Using PCA and k-means clustering, we group 1,954 distinct tropes into 15 semantically interpretable clusters. Chi-square analyses show that the six main characters are unevenly distributed across these clusters, with character-specific trope profiles that are broadly consistent with their established narrative identities. Finally, we project trope clusters into the ousiometric power-danger space to examine their semantic organization. The results show that "Physical and Sexual Comedy" occupies a region associated with relatively high danger, while "Revelation, Surprise, and Reaction" occupies a region associated with relatively high power. Overall, our work demonstrates a way to operationalize trope measurement and shows that identifiable trope clusters can provide holistic "distant reading" descriptions of characters and stories.

==> settings/assignment.header.tex <==
\begin{center}
  \raisebox{-22pt}{\includegraphics[width=0.2\textwidth]{pocslogo002.pdf}}~\begin{tabular}{c}
    \textbf{\coursename}\\
    \textbf{\fullcoursenumber}\\
    \textbf{\fullinstitution, \season\ \courseyear}\\
    %%      \textbf{{\solutionsto}Assignment \assignmentnumtext\ $\bullet$ code name: \codename}
    \textbf{{\solutionsto}Assignment \assignmentnumtext} \\
    \textbf{\codename}      
  \end{tabular}
\end{center}

\ifthenelse{\not\boolean{solutionsboolean}}
{
  {\small
    %% \textbf{Dispersed:} \outdate, \courseyear.\\
    \textbf{Due:} \duedate \\
%%    \textbf{Due:} \duedate, \courseyear.\\
    %% \textbf{Sections covered:} \sectionscovered.
%%    \textbf{Relevant clips, episodes, and slides} are listed on the assignment's page:
    \href{\coursewebsite/assignments/\assignmentnumtext/}{\coursewebsite/assignments/\assignmentnumtext/}\\
    \textit{Some useful reminders:}\\
    \textbf{Deliverator:} \myname\ (contact through Teams)\\ %% \myemail
    \textbf{Assistant Deliverator:} \taname\ (contact through Teams) \\ %% \taemail
    \textbf{Office:} The Ether \\
%%    \textbf{Office:} \officelocation \\ 
    \textbf{Office hours:} \officehours \\
    \textbf{Course website:} \href{\coursewebsite}{\coursewebsitetext}
    \textbf{Overleaf:} LaTeX templates and settings for all assignments are
    available at \overleafurl.
%%    \textbf{Bonus course notes:}
%%    \href{\coursewebsite/docs/dewhurst-pocs-notes.pdf}{\coursewebsitetext/docs/dewhurst-pocs-notes.pdf}
  }

\medskip

\hrule

{\small
All parts are worth 3 points unless marked otherwise.
Please show all your workingses clearly and list the names of
others with whom you \sout{conspired} collaborated.

%% Please obey the basic life rule: Never use Excel.
%% Or any Microsoft product except maybe Xbox (which sadly will likely not help you here). Okay, Teams is not that bad. Back to the point:
For coding, we recommend you improve your skills with Python, R, and/or Julia. The (evil) Deliverator uses (evil) Matlab.

Graduate students are requested to use \LaTeX\ (or related \TeX\
variant). If you are new to \LaTeX, please endeavor to submit at least $n$ questions per assignment in \LaTeX, where $n$ is the assignment number.

\textbf{Assignment submission:}

Via Brightspace or other preferred death vortex.

%% \textbf{email submission:}
%% If Blackboard is not set up:\\
%% 1. Please send to both the Assistant Deliverator \taname\ via direct message on Teams.\\
%% 2. PDF only! Please name your file as follows (where the number is to be padded
%% by a 0 if less than 10 and names are all lowercase):
%% \texttt{CSYS300assignment\%02d\$firstname-\$lastname.pdf}
%% as in 
%%\texttt{CSYS300assignment06michael-palin.pdf}

}

\medskip
\medskip

\hrule

\medskip
}
{} % do nothing


==> settings/settings.assignments-all.tex <==
\newboolean{solutionsboolean}
\newboolean{videoboolean}

\urlstyle{same}

\usepackage{comment}

\usepackage[usenames]{color}
\newcommand{\tc}[2]{\textcolor{#1}{#2}}
\newcommand{\tcn}[2]{\color[named]{#1}{#2}}
\definecolor{olivegreen}{rgb}{0.33333,.41961,0.18431}
\definecolor{forestgreen}{rgb}{0.13333,.5451,0.13333}
\definecolor{lightgrey}{rgb}{0.7,0.7,0.7}
\definecolor{grey}{rgb}{0.5,0.5,0.5}
\definecolor{darkgrey}{rgb}{0.3,0.3,0.3}
\definecolor{verydarkgrey}{rgb}{0.1,0.1,0.1}

\usepackage{etoolbox}


\newcommand{\solutionstart}{\textbf{Solution:}}
\newcommand{\solutionend}{\hfill $\square$}

\usepackage{environ}

\NewEnviron{solution}{
  %% $\ulcorner$ \hfill $\urcorner$ \\

  \ifthenelse{\boolean{solutionsboolean}}{
    \normalcolor

    \solutionstart
    % \marginpar{\rule[-17.5mm]{1pt}{20mm}}
    \BODY
    \solutionend
  }

%%  \color{darkgrey}
  % $\llcorner$ \hfill $\lrcorner$ 
  % $\boxplus$
}[]




\usepackage{marvosym}

\newcommand{\pleasesubmitprojectdraft}{
  \ifthenelse{\not\boolean{solutionsboolean}}{
    {\small
    \textbf{Please submit your project's current draft}
    in pdf format via Brightspace by the same time specified for this assignment.
    For teams, please list all team member names clearly at the start.
    
%%     Please use this file name format (all lowercase after CSYS):\\
%%     \texttt{{\fullcoursenumbertext}project-\$firstname-\$lastname-YYYY-MM-DD.pdf}
%%     as in 
%%     \texttt{{\fullcoursenumbertext}project-lisa-simpson-1989-12-17.pdf}
%%     where the date is the date of submission (and not, say, your birthdate).
    }
    \medskip

    \hrule

    \medskip
  }{}
}

\usepackage{cancel}
\usepackage{verbatim}


\newcommand{\alert}[1]{#1}
\newcommand{\alertb}[1]{#1}


\newcommand{\tfline}{\underline{\mbox{\qquad \ }}.}


\newcommand{\veck}{\vec{k}}
%% \newcommand{\veck}{\mathbf{k}}

\newcommand{\infprob}{B}
\newcommand{\gainratio}{\mathbf{R}}

\newcommand{\undmark}{\rm und}
\newcommand{\dirmark}{\rm dir}

\newcommand{\bidmark}{\rm u}
\newcommand{\inmark}{\rm i}
\newcommand{\outmark}{\rm o}

\newcommand{\kin}{k_{\inmark}}
\newcommand{\kout}{k_{\outmark}}
\newcommand{\kbid}{k_{\bidmark}}

\newcommand{\jin}{j_{\inmark}}
\newcommand{\jout}{j_{\outmark}}
\newcommand{\jbid}{j_{\bidmark}}


\newcommand{\Probdir}{P^{(\rm \dirmark)}}

\newcommand{\Probin}{P^{(\rm \inmark)}}
\newcommand{\Probout}{P^{(\rm \outmark)}}
\newcommand{\Probbid}{P^{(\rm \bidmark)}}

\newcommand{\nodetype}{\kin,\kout,\kbid}

\newcommand{\edgetype}{\veck\, |\, \veck'}
\newcommand{\edgetypescript}{\veck\veck'}

%% \newcommand{\probfc}{\chi}
\newcommand{\probfc}{Q}

%% \newcommand{\edgetype}{\vec{k};\vec{\alpha}\, |\, \vec{k}';\vec{\alpha}'}
%% \newcommand{\edgetypescript}{\vec{k}\vec{\alpha}\vec{k}'\vec{\alpha}'}

\newcommand{\indrspfn}{h}
\newcommand{\rspfn}{H}


==> settings/settings.assignments.tex <==
\newcommand{\solutioncolorswitch}{\color{darkgrey}}

%% \newcommand{\solution}[1]
%% {
%% % $\ulcorner$ \hfill $\urcorner$ \\
%% 
%% \normalcolor
%% 
%% \textbf{Solution:} 
%% % \marginpar{\rule[-17.5mm]{1pt}{20mm}}
%% \color{black}{#1}
%% % $\llcorner$ \hfill $\lrcorner$ 
%% % $\boxplus$
%% \hfill $\square$
%% 
%% \color{darkgrey}
%% 
%% }



\newcommand{\solutionsto}{Solutions to }

\setboolean{solutionsboolean}{true}
\setboolean{videoboolean}{false}

\newcommand{\assignmentsonly}[1]{}


==> settings/settings.course.tex <==
%% volume one and two switches throughout

\newcommand{\coursename}{Principles of Complex Systems, Vols. 1, 2, \& 3D}
\newcommand{\courseacronym}{PoCS}
\newcommand{\courseuniverse}{The PoCSverse}
\newcommand{\courseacronymlc}{pocs}
\newcommand{\courseacronymcompact}{PoCS}
\newcommand{\coursetag}{pocsverse}
\newcommand{\fullcoursenumber}{CSYS/MATH 6701, 6713, \& a pretend number}

\newcommand{\coursenamevolumeone}{Principles of Complex Systems. Vol. 1}
\newcommand{\coursenamevolumetwo}{Principles of Complex Systems. Vol. 2}
\newcommand{\coursenamevolumethree}{Principles of Complex Systems, Vol. 3D}
%% \newcommand{\coursenamevolumethree}{Advanced Topics in Complex Systems}
%% \newcommand{\coursenamevolumethree}{Advanced Topics in Complex Systems: Ousiometrics, Telegnomics, and Stories}

\newcommand{\coursenamevolumeoneshort}{Principles Complex Systems, Vol 1.}
\newcommand{\coursenamevolumetwoshort}{Principles Complex Systems, Vol 2.}
\newcommand{\coursenamevolumethreeshort}{Principles Complex Systems, Vol. 3D}

\newcommand{\coursenumber}{6701}
\newcommand{\coursesection}{A}
\newcommand{\computernumber}{93127/93833/94109}
\newcommand{\fullcoursenumbertext}{CSYS\coursenumber}

\newcommand{\coursenumbervolumeone}{6701}
\newcommand{\coursesectionvolumeone}{A}
\newcommand{\computernumbervolumeone}{93127/93833/94109}
\newcommand{\fullcoursenumbertextvolumeone}{CSYS\coursenumber}

\newcommand{\coursenumbervolumetwo}{6713}
\newcommand{\coursesectionvolumetwo}{A}
\newcommand{\computernumbervolumetwo}{}
\newcommand{\fullcoursenumbertextvolumetwo}{CSYS\coursenumbervolumetwo}

\newcommand{\coursenumbervolumethree}{Imaginary}
\newcommand{\coursesectionvolumethree}{A}
\newcommand{\computernumbervolumethree}{Imaginary}
\newcommand{\fullcoursenumbertextvolumethree}{CSYS\coursenumbervolumethree}

\newcommand{\courseseason}{18}

\newcommand{\pocsvoltwostartassignment}{12}

%% %% vestigial
%% %% randomizer for course nickname
%% \perlnewcommand{\coursenickname}{
%%   @nicknames = ('Complex Networks: Revenge of the PoCS',
%%   'PoCS: Complex Networks Edition',
%%   'CocoNuTS',
%%   'CoNKs',
%%   'sCoNes',
%%   'Complex Networks: The PoCS Strikes Back',
%%   'Monk owl excerpts',
%%   'Next PoCS: Elk Worm',
%%   'Ex-crow pelts monk',
%%   'Plot: Corms Knew Ex',
%%   'Plot: Ex mocks Wren',
%%   'Plot: Ox wrecks men',
%%   );
%%   return $nicknames[rand @nicknames];
%% }

%% for assignments
%% 2023--2024
\newcommand{\overleafurl}{https://www.overleaf.com/read/tsxfwwmwdgxj}

%% \newcommand{\overleafurl}{https://www.overleaf.com/project/64f28b090d0139d74fa4043e}

\newcommand{\teamsurl}{https://teams.microsoft.com/l/channel/19\%3a4d62bc9c659c4717a884f02b54546f8d\%40thread.tacv2/General?groupId=24e0c156-f786-4d99-bbdd-5d4489db90e7\&tenantId=1c177758-4d6b-43dc-aaeb-3b9c42562967}
\newcommand{\slackurl}{}

\newcommand{\teamsurlsemesterone}{}
\newcommand{\teamsurlsemestertwo}{}

\newcommand{\courseyear}{2023}
\newcommand{\coursemonth}{08}
\newcommand{\season}{Fall}

\newcommand{\courseyearfirsthalf}{2023}
\newcommand{\coursemonthfirsthalf}{08}
\newcommand{\seasonfirsthalf}{Fall}

\newcommand{\courseyearsecondhalf}{2024}
\newcommand{\coursemonthsecondhalf}{01}
\newcommand{\seasonsecondhalf}{Spring}

\newcommand{\courseyearthirdhalf}{2023}
\newcommand{\coursemonththirdhalf}{08}
\newcommand{\seasonthirdhalf}{Fall}

\newcommand{\secondhalffirstassignmentnum}{15}

\newcommand{\lastcourseyear}{2022}
\newcommand{\lastcoursemonth}{08}

\newcommand{\logosuffix}{logo.pdf}
\newcommand{\courselogo}{\courseacronymlc\logosuffix}

\newcommand{\lectureroom}{Mann Hall, 102C}
\newcommand{\meetingtimes}{10:05 am to 11:20 am}
\newcommand{\lecturestarttime}{10:05 am}

\newcommand{\lectureroomvolumeone}{Mann Hall, 102C}
\newcommand{\meetingtimesvolumeone}{10:05 am to 11:20 am}
\newcommand{\lecturestarttimevolumeone}{10:05 am}

\newcommand{\lectureroomvolumetwo}{Lafayette 210}
\newcommand{\meetingtimesvolumetwo}{10:05 am to 11:20 am}
\newcommand{\lecturestarttimevolumetwo}{10:05 am}

\newcommand{\lectureroomvolumethree}{Vermont Complex Systems Center}
\newcommand{\meetingtimesvolumethree}{TBA}
\newcommand{\lecturestarttimevolumethree}{TBA}


\newcommand{\fullinstitution}{University of Vermont}
\newcommand{\institution}{UVM}

\newcommand{\coursehandle}{@pocsvox}
\newcommand{\coursetwitterhandlelink}{\href{https://twitter.com/\coursehandle}{\coursehandle}}
\newcommand{\coursehashtag}{\#\season\courseacronymcompact\courseyear}


\newcommand{\courseprefix}{\courseyearfirsthalf-\courseyearsecondhalf\coursetag}


%% websites
\newcommand{\institutionwebsite}{https://pdodds.w3.uvm.edu}
\newcommand{\mywebsitehomedir}{}

%% \newcommand{\visitinginstitutionwebsite}{http://www.massmutual.com}

%% \newcommand{\mywebsitehomedirtext}{$\sim$pdodds}
%% \newcommand{\mywebsitehomedirtext}{{\textasciitilde{}}pdodds}
\newcommand{\mywebsitehomedirtext}{}


\newcommand{\mywebsite}{\institutionwebsite/\mywebsitehomedir}
\newcommand{\mywebsiteresearch}{\institutionwebsite/research}
\newcommand{\mywebsitevideos}{\institutionwebsite/videos}
\newcommand{\myemailaddress}{peter.dodds+pocs@uvm.edu}
\newcommand{\mytwitterhandle}{@peterdodds}
\newcommand{\mytwitterhandlelink}{\href{https://twitter.com/\mytwitterhandle}{\mytwitterhandle}}

\newcommand{\teachingsite}{\institutionwebsite/teaching}
\newcommand{\coursewebsite}{\teachingsite/courses/\courseprefix}
\newcommand{\coursewebsitetext}{\institutionwebsite/teaching/courses/\courseprefix}

%% slides

%% \newcommand{\defaultslidebackground}{slidebackground-vintage_grid.jpg}
\newcommand{\defaultslidebackground}{figures/local/slidebackground-vintage_grid-faded.jpg}

%% figures

\newcommand{\papersdir}{\institutionwebsite/\mywebsitehomedir/research/papers/others}


%% header
 \newcommand{\courseheader}{ \makebox[\textwidth]{
\raisebox{-25pt}{\includegraphics[width=0.35\textwidth]{pocslogo100.pdf}}%
\qquad\qquad
\hfill \normalsize%
\begin{tabular}{r}
  \textbf{\large \coursename} \\
  \coursetwitterhandlelink\\
  \fullcoursenumber\\
  Unreliable Deliverator: \myname\\
%%  \meetingtimes\ in \lectureroom\\
  \bigskip
\end{tabular}\newline
   }
   \href{\coursewebsite}{\coursewebsitetext/}
   \bigskip
   \hrule
}
%% text

\newcommand{\sourcematerial}{Journal papers and book excerpts}
\newcommand{\textbook}{No official textbook}

\newcommand{\officelocation}{The Ether and/or Innovation, fourth floor}
%% \newcommand{\officelocation}{To be disclosed}

\newcommand{\officehours}{See Teams calendar}
%% \newcommand{\officehours}{Tuesdays, 3:00 to 4:00 pm on Teams}
%% Tuesdays, 12 to 12:50 pm; Wednesdays, 1:15 pm to 2:05 pm; Thursdays, 12 to 12:50 pm; all scheduled on Teams}

%% \newcommand{\officehours}{To be emphatically determined through a democratic process}
%% \newcommand{\officehours}{Maybe: 11:40 am to 11:55 am, Tuesday and Thursday, and 2:00 pm to 4:00 pm, Wednesday}


\newcommand{\finalexamdatelocation}{%%
  Friday, December 14, 8:30 am, \lectureroom.
}
\newcommand{\finalexamdatelocationvolumeone}{%%
  Friday, December 14, 8:30 am, \lectureroom.
}
\newcommand{\finalexamdatelocationvolumetwo}{%%
  TBD, \lectureroom.
}
\newcommand{\finalexamdatelocationvolumethree}{%%
  TBD, \lectureroom.
}

\newcommand{\myname}{\href{\mywebsite}{Prof. Peter Sheridan Dodds}}
\newcommand{\myemail}{peter.dodds@uvm.edu}

\newcommand{\showrunnername}{\href{\mywebsite}{Prof. Peter Sheridan Dodds}}
\newcommand{\showrunnertwitterhandle}{@peterdodds}
\newcommand{\myshowrunnertwitterhandlelink}{\href{https://twitter.com/\myshowrunnertwitterhandle}{\myshowrunnertwitterhandle}}

\newcommand{\taname}{\href{\mywebsite}{Chris O'Neil}}
\newcommand{\taemail}{christopher.oneil@uvm.edu}

\newcommand{\lectureschedule}{
  \begin{tabular}{|p{.22\textwidth}|p{.3\textwidth}|p{.3\textwidth}|}
    \hline
    \textbf{Week \#}& \textbf{Tuesday} & \textbf{Thursday} \\
    \hline
    1 %% (8/31 and 9/02) 
    &
    Overview; Fundamentals: \newline The Complexity Manifesto 
    &
    Scaling
    \\
    \hline
    2 %% (9/07 and 9/09)
    &
    Power-law size distributions 
    &
    Zipf's law;
    Fundamentals: 
    \\
    \hline
    3 %% (9/14 and 9/16)       
    &
    Allotaxonometry
    &
    Power-law mechanisms: Randomness 
    \\
    \hline
    4 %% (9/21 and 9/23)
    &
    Power-law mechanisms: \newline Variable Transformation  
    &
    Power-law mechanisms: \newline The Rich-Get-Richer 
    \\
    \hline
    5 %% (9/28 and 9/30)
    &
    Power-law mechanisms: Optimization
    &
    Fundamentals:
    Statistical Mechanics;
    \\
    \hline                                                                        
    6 %% (10/05 and 10/07)
    &
    Robustness and Fragility 
    &
    Optimal distribution networks
    \\
    \hline
    7 %% (10/12 and 10/14)
    & 
    Fundamentals:
    Data, Emergence, Limits to
    Understanding;
    &
    First project presentations
    \\
    \hline                                                                        
    8 %% (10/19 and 10/21)
    &
    Complex networks: Introduction\newline Basics and Examples 
    &
    Complex networks: Key Properties\newline Generalized random networks
    \\
    \hline                                                                        
    9 %% (10/26 and 10/28)
%%    & Project presentations$^{\dagger}$ 
    &
    Complex networks:\newline Small-world networks  
    &
    Complex networks:\newline Small-world networks  
    \\
    \hline
    10 %% (11/02 and 11/04)
    &
    Complex networks:\newline Scale-free networks 
    &
    Contagion: Introduction 
    \\
    \hline
    11 %% (11/09 and 11/11)
    &
    The Unpredictability of Pandemics
    &
    COVID-19
    \\
    \hline
    12 %% (11/16 and 11/18)
    &
    Social contagion
    &
    Social Contagion 
    \\
    \hline                                                                        
    13 %% (11/23 and 11/25)
    &
    Thanksgiving 
    &
    Thanksgiving 
    \\
    \hline
    14 %% (11/30 and 12/02)
    &
    Social Contagion 
    &
    Voting, Success, Fame
    \\
    \hline
    15 %% (12/07 and 12/09)
    &
    Stories 
    &
    The Big Story: Complexification
    \\
    \hline
  \end{tabular}\\
  \smallskip
%%  $\dagger$: 3-4 minutes each + 1 or 2 questions;

  %% $^\ddagger$: 3-4 minutes each + 1 or 2 questions.
  %% Guest lecture: Jake Williams, Zipf's law and Simon's model for phrases \\               
}

\newcommand{\importantdates}{
  \begin{enumerate}
  \item
    Classes run from Monday, August 28 to Friday, December 8.
  \item
    Add/Drop, Audit, Pass/No Pass deadline---Monday, September 11.
  \item
    Last day to withdraw---Monday, October 30 (Sadness!).
  \item
    Reading and Exam period---Saturday, December 9 to Friday, December 15.
  \end{enumerate}
}

\newcommand{\importantdatesvolumeone}{\importantdates}

\newcommand{\importantdatesvolumetwo}{
  \begin{enumerate}
  \item
    Classes run from Monday, January 16 to Friday, May 3.
  \item
    Add/Drop, Audit, Pass/No Pass deadline---Monday, January 29.
  \item
    No class on Tuesday, March 5 (Town Meeting Day Recess).
  \item
    Spring recess, March 11 to 15.
  \item
    Last day to \sout{escape} withdraw---Monday, April 1.
  \item
    Reading and Exam period---Saturday, May 4 to Friday, May 10.
  \end{enumerate}
}



\newcommand{\standardpolicies}{
\textbf{Do} check the course's main website, Teams, and the course's Twitter account, \coursehandle, for updates regarding the course.

\textbf{Academic assistance:} Anyone who requires assistance in any way (as per the ACCESS program
or due to athletic endeavors), please see or contact me as soon as possible.

\textbf{Being good people:} 
In class there will be no unnecessary electronic gadgetry,
no cell phones, no beeping, no text messaging, etc.  
You really just need your brain, some paper, and a writing implement.
%% Those who beep in an annoying fashion will be fined one organic banana by the lecturer.
I encourage you to use the course's Teams site
to ask questions, share ideas, comments, etc., about the class and assignments
but request that you please do so in a respectful fashion.
Moreover, all interactions with classmates during lectures and office hours or
in any way related to being part of PoCS should be respectful.
As in all UVM classes,
\textbf{Academic honesty} will be expected and departures will 
be dealt with appropriately.
We will follow UVM's community standards
and guidelines. See \url{https://www.uvm.edu/cses/}.

\textbf{Late policy:} Unless in the case of an emergency (a real one) or if
an absence has been predeclared and a make-up version
sorted out, assignments that are not turned in on time or tests that are not 
attended will be given 0\%.

\textbf{Grades:}
\begin{tabular}{|ll|ll|ll|ll|}
  \hline
  A+ & 97--100 & B+ & 87--89 & C+ & 77--79 & D+ & 67--69 \\
  A  & 93--96  & B  & 83--86 & C  & 73--76 & D  & 63--66 \\
  A- & 90--92  & B- & 80--82 & C- & 70--72 & D- & 60--62 \\
  \hline
\end{tabular}
}




==> settings/settings.general.tex <==
\usepackage{media9}

\usepackage{censor}


%% set current time
\usepackage{datetime}
%% \yyyymmdddate
\newtimeformat{mytime}{\twodigit{\THEHOURXII}:\twodigit{\THEMINUTE}}
\settimeformat{mytime}
\newdateformat{mydate}{\dayofweekname{\THEDAY}{\THEMONTH}{\THEYEAR}, \monthname\ \THEDAY, \THEYEAR}
\mydate

%% for toggling solutions
\usepackage{environ}

%% eh
\newcommand{\pocsvoloneonly}[1]{}
\newcommand{\pocsvoltwoonly}[1]{}

%% links
\usepackage{url}
%% url style
\urlstyle{same}

%% allow hyphenation for urls with long many-hyphenated strings
\PassOptionsToPackage{hyphens}{url}\usepackage{hyperref}
\makeatletter
\g@addto@macro{\UrlBreaks}{\UrlOrds}
\makeatother

\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=grey,
    citecolor=todoblue,
    filecolor=grey,
    urlcolor=grey,
    breaklinks=true,
}

%% exciting emphasis action
\usepackage{ulem}
%% note that to allow linebreaking,
%% separate words as \dashuline{the\ slithy\ tove};
%% it may be necessary to format arguments 
%% in this way (e.g., section headings)
%% base html for documents (lectures and assignments)

\usepackage{cprotect}
%% code snippets
%% http://stackoverflow.com/questions/3175105/how-to-insert-code-into-a-latex-doc
\usepackage{listings}
\usepackage[numbered]{matlab-prettifier}

%% showing latex along with output
%% https://tex.stackexchange.com/questions/110349/any-way-to-show-latex-example-code-and-execute-it
\usepackage{showexpl}

%% use this for functions:
%% \begin{lstlisting}[style=Matlab-editor]
%% \end{lstlisting}\begin{verbatim}

\usepackage{fontawesome}


\definecolor{todoblue}{RGB}{0, 91, 187}
\newcommand{\todo}[1]{\noindent\textcolor{todoblue}{{$\Box$ #1}}}

\newcommand{\wikilink}[1]{\href{#1}{\tc{grey}{\faExternalLink}}}
\newcommand{\wordwikilink}[2]{\href{#1}{\tc{grey}{\dashuline{#2}~\faExternalLink}}}
\newcommand{\wordwikilinklong}[2]{\href{#1}{\tc{grey}{\url{#2}~\faExternalLink}}}



\newcommand{\Prob}{\mathbf{Pr}}

\newcommand{\degree}{\, \circ}
\newcommand{\tempf}[1]{${#1}^{\degree}F$}
\newcommand{\tempc}[1]{${#1}^{\degree}C$}

\newcommand{\avg}[1]{\left\langle#1\right\rangle}
\newcommand{\tavg}[1]{\langle#1\rangle}

\newcommand{\LavgHa}[2]{\tavg{L_{#1,#2}}}
\newcommand{\LavgHaN}[2]{\tavg{L_{#1,#2}}}
\newcommand{\Lavg}{\tavg{L}}

\newcommand{\sindex}[1]{}
\newcommand{\nindex}[1]{}

\newcommand{\etal}{\textit{et al.}}
\newcommand{\www}[1]{\url{#1}}
\newcommand{\req}[1]{(\ref{#1})}
\newcommand{\Req}[1]{Eq.~(\ref{#1})}


\newcommand{\yes}{}
\newcommand{\no}{}
\newcommand{\tbf}{\textbf}
\newcommand{\tit}{\textit}

\newcommand{\stirlingnumber}[2]{\genfrac{\{}{\}}{0pt}{}{#1}{#2}}


\newcommand{\dee}[1]{\mbox{d}#1}
\newcommand{\pdiff}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\partialdiff}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\partialdiffsq}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\pdiffsq}[2]{\frac{\partial^2 #1}{{\partial #2}^2}}
\newcommand{\diff}[2]{\frac{{\rm d}#1}{{\rm d}#2}}
\newcommand{\diffsq}[2]{\frac{{\rm d}^{2}#1}{{\rm d} {#2}^2}}
\newcommand{\tdiff}[2]{\mbox{d} #1/\mbox{d} #2}
\newcommand{\tdiffsq}[2]{\mbox{d}^{2} #1/\mbox{d} {#2}^2}
\newcommand{\tpdiff}[2]{\partial #1/\partial #2}
\newcommand{\tpdiffsq}[2]{\partial^2 #1/\partial {#2}^2}
\newcommand{\postdee}[1]{\,\mbox{d}#1}


%% binomials
\newcommand{\mybinom}[2]{\Bigl(\begin{array}{@{}c@{}}#1\\#2\end{array}\Bigr)}

%% half
\newcommand{\half}{\frac{1}{2}}



% \newcommand{\avgSL}{\bar{L}_{\rm s}}
\newcommand{\avgSL}{\tavg{l_{\rm s}}}


\newcommand{\fplus}{f_{+}}
\newcommand{\fminus}{f_{-}}
\newcommand{\aplus}{a_{+}}
\newcommand{\aminus}{a_{-}}



% \newcommand{\kstar}{d^{\ast}}
% \newcommand{\kstari}{k_i^\ast}
\newcommand{\kstar}{d^\ast}
\newcommand{\kstari}{d_i^\ast}

\newcommand{\dstar}{d^\ast}
\newcommand{\dstari}{d_i^\ast}

\newcommand{\phifix}{{\phi^{\ast}}}
\newcommand{\phifixc}{{\phi_c^{\ast}}}
\newcommand{\phifixb}{{\phi_b^{\ast}}}

\newcommand{\Gfun}{G}


\newcommand{\dstardist}{g}
\newcommand{\dosedist}{f}
\newcommand{\dosedistk}{f^{k\star}}

\newcommand{\erdosrenyi}{Erd\"{o}s-R\'{e}nyi}

\newcommand{\meandegree}{z}

\newcommand{\stateA}{0}
\newcommand{\stateB}{1}

\newcommand{\phiA}{\phi_0}
\newcommand{\phiB}{\phi_1}

\newcommand{\phiup}{\phi^{\rm up}}
\newcommand{\phidown}{\phi^{\rm down}}
\newcommand{\phiupi}{\phi_i^{\rm up}}
\newcommand{\phidowni}{\phi_i^{\rm down}}

\newcommand{\phihomog}{\phi_{\rm h}}
\newcommand{\phiuphomog}{\phi_{\rm h}^{\rm up}}

\newcommand{\vcluster}{\mathcal{V}_{\rm max}}
\newcommand{\initset}{\mathcal{A}}

\newcommand{\avggroupdeg}{\tavg{k_{\rm group}}}

\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}


%% scaling

\newcommand{\xmin}{x_\textnormal{min}}
\newcommand{\xmax}{x_\textnormal{max}}


%% video hints:

\newcommand{\videohint}[2]{
  \ifthenelse{\boolean{videoboolean}}{
 \begin{minipage}{1.0\linewidth}
   \textbf{Hint---}#2:\\
   \includemedia[
   width=1\linewidth,height=0.5625\linewidth,
   activate=pageopen,
   flashvars={
     modestbranding=0 % no YT logo in control bar
     &autoplay=0
     &fs=1
     &autohide=1 % controlbar autohide
     &showinfo=0 % no title and other info before start
     % &rel=0
     % &rel=0 % no related videos after end
   }
   ]
   {}
   {http://www.youtube.com/watch?v=#1}\\
   Direct link: \url{http://www.youtube.com/watch?v=#1}
%   {http://www.youtube.com/watch?v=#1?rel=0}\\
%   Direct link: \url{http://www.youtube.com/watch?v=#1?rel=0}
   %% \url{http://www.youtube.com/watch?v=#1?rel=0}
 \end{minipage}
  }
  {
    \textbf{Hint---#2}: \url{http://www.youtube.com/watch?v=#1}
%%    \textbf{Hint---#2}: \url{http://www.youtube.com/watch?v=#1?rel=0}
  }
}

\newcommand{\videohelp}[7]{
  %% youtube embeds no longer work
  %% 
%%   %% #1: video
%%   %% #2: title
%%   %% #3: start
%%   %% #4: end (only works in embed)
%%   %% #5: video length
  \ifthenelse{\boolean{videoboolean}}{
    \begin{minipage}{1.0\linewidth}
      \textbf{Help---}#2 (runs from #5 to #6, length #7):\\
      \includemedia[
      width=1\linewidth,height=0.5625\linewidth,
      activate=pageopen,
      flashvars={
        modestbranding=0 % no YT logo in control bar
        &autoplay=0
        &fs=1
        &autohide=0 % controlbar autohide
        &showinfo=0 % no title and other info before start
        &start=#3
        &end=#4
%        &rel=0
        % &rel=0 % no related videos after end
      }
      ]
      {}
      %% {http://www.youtube.com/watch?v=#1?rel=0&start=#3&end=#4}\\
      {http://www.youtube.com/watch?v=#1?start=#3&end=#4}\\
      \tc{grey}{Note: Video embed only works in Adobe Reader. Direct link:}\\
      \tc{grey}{\url{http://www.youtube.com/watch?v=#1?\&start=#3\&end=#4}}
%%      \tc{grey}{\url{http://www.youtube.com/watch?v=#1\&rel=0\&start=#3\&end=#4}}
      %% \url{http://www.youtube.com/watch?v=#1?start=#3&end=#4&rel=0}
    \end{minipage}
  }
  {
    \textbf{Help---#2} (runs from #5 to #6, length #7): \url{http://www.youtube.com/watch?v=#1?start=#3\&end=#4}
%%    \textbf{Help---#2} (runs from #5 to #6, length #7): \url{http://www.youtube.com/watch?v=#1\?rel=0\&start=#3\&end=#4}
  }
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% matrices
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\m}[1]{\mathbf{#1}}

\newcommand{\colvec}[1]{
\left[
  \begin{array}{c}
    #1
  \end{array}
\right]
}

\newcommand{\rowop}[3]{
  {
    \scriptsize
    \begin{array}{c}
      \mbox{\Large $\leadsto$} \\
      \mbox{#1' =} \\
      \mbox{#1 -} \\ 
      \mbox{#2 #3} \\
    \end{array}
  }
}

\newcommand{\rowoptwobytwo}[3]{
  {
    \scriptsize
    \begin{array}{c}
      \mbox{\Large $\leadsto$} \\
      \mbox{#1'} 
      \mbox{= #1 -}
      \mbox{#2 #3} \\
    \end{array}
  }
}

\newcommand{\rowopeq}[3]{
  {
    \scriptsize
    \begin{array}{c}
      \mbox{\Large =} \\
      \left\lgroup
      \mbox{\tiny
        \begin{tabular}{c}
          #1' =  \\
          #1 - #2 #3 \\
        \end{tabular}
    }
      \right\rgroup
    \end{array}
  }
}

\newcommand{\rowswapeq}[2]{
  {
    \scriptsize
    \begin{array}{c}
      \mbox{\large =} \\
      \left\lgroup
      \mbox{\tiny
          #1 $\leftrightarrow$ #2
        }
      \right\rgroup
    \end{array}
  }
}

\newcommand{\rowdiv}[2]{
  {
    \scriptsize
    \begin{array}{c}
      \mbox{\Large $\leadsto$} \\
      \mbox{#1' =} \\
      \mbox{#1/(#2)} \\ 
    \end{array}
  }
}

\newcommand{\rowdivthreebythree}[3]{
  {
    \scriptsize
    \begin{array}{c}
      \mbox{\Large $\leadsto$} \\
      \mbox{row 1'} = \mbox{row 1/(#1)}\\
      \mbox{row 2'} = \mbox{row 2/(#2)}\\
      \mbox{row 3'} = \mbox{row 3/(#3)}\\
    \end{array}
  }
}


\newcommand{\rowdivtwobytwo}[2]{
  {
    \scriptsize
    \begin{array}{c}
      \mbox{\Large $\leadsto$} \\
      \mbox{row 1'} = \mbox{row 1/(#1)}\\
      \mbox{row 2'} = \mbox{row 2/(#2)}\\
    \end{array}
  }
}

\newcommand{\rowdivtwobytwoeq}[2]{
  {
    \scriptsize
    \begin{array}{c}
      \mbox{\Large =} \\
      \mbox{row 1'} = \mbox{row 1/(#1)}\\
      \mbox{row 2'} = \mbox{row 2/(#2)}\\
    \end{array}
  }
}

\newcommand{\rowdivthreebythreeeqR}[3]{
  {
    \scriptsize
    \begin{array}{c}
      \mbox{\Large =} \\
      \mbox{R1'} = \mbox{R1/(#1)}\\
      \mbox{R2'} = \mbox{R2/(#2)}\\
      \mbox{R3'} = \mbox{R3/(#3)}\\
    \end{array}
  }
}


\newcommand{\rowdivtwobytwoeqR}[2]{
  {
    \scriptsize
    \begin{array}{c}
      \mbox{\Large =} \\
      \mbox{R1'} = \mbox{R1/(#1)}\\
      \mbox{R2'} = \mbox{R2/(#2)}\\
    \end{array}
  }
}


\newcommand{\rowonediv}[1]{
  {
    \scriptsize
    \begin{array}{c}
      \mbox{\Large $\leadsto$} \\
      \mbox{row 1'} = \mbox{row 1/#1}\\
    \end{array}
  }
}

\newcommand{\mymatrix}[2]{
  \left[
  \begin{array}{#1}
    #2
  \end{array}
  \right]
}

%% \newcommand{\matrix}[1]{\mathbf{#1}}
\newcommand{\textmatrix}[1]{#1}

%% \renewcommand{\m}[1]{\mathbf{#1}}

\newcommand{\Axb}{\textmatrix{A}\vec{x}=\vec{b}}
\newcommand{\Axzero}{\textmatrix{A}\vec{x}=\vec{0}}
\newcommand{\A}{\textmatrix{A}}
\newcommand{\AT}{\textmatrix{A}^{\rm T}}
\newcommand{\CA}{C(\textmatrix{A})}
\newcommand{\NA}{N(\textmatrix{A})}
\newcommand{\CAT}{C(\textmatrix{A}^{\rm T})}
\newcommand{\NAT}{N(\textmatrix{A}^{\rm T})}

\newcommand{\I}{\textmatrix{I}}
\newcommand{\R}{\textmatrix{R}}

\newcommand{\augAb}{[\A \, | \, \vec{b} \, ]}

\newcommand{\rref}[1]{\R_{#1}}

\newcommand{\lmat}{\left[
\begin{array}
}
\newcommand{\rmat}{\end{array}
\right]
}



%% girl born on a tuesday problem
\newcommand{\girl}{G}
\newcommand{\boy}{B}
\newcommand{\girltues}{G_{\textnormal{Tue}}}


%% entropy
\newcommand{\Hrenyi}[1]{H^{\textnormal{(R)}}_{#1}}
\newcommand{\Htsallis}[1]{H^{\textnormal{(T)}}_{#1}}
%% branching networks

%% river networks
\newcommand{\rhodd}{\rho_{\rm dd}} % drainage density
\newcommand{\msl}{\ell} % main stream length
%% \newcommand{\okell}{{l^{\mbox{\scriptsize{(s)}}}}}
%% \newcommand{\okellsnum}[1]{l_{#1}^{\mathrm{\, (s)}}}
\newcommand{\okell}{s}
\newcommand{\okellsnum}[1]{s_{#1}}

\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}

\newcommand{\Tmunu}{T_{\mu,\nu}}

\newcommand{\rpartition}[7]{%
  #1(#2\!\!#3,#4\!\!#5#6#7)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% optimal forks (Murray's law)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\rparent}{r_{\textnormal{parent}}}
\newcommand{\rchilda}{r_{\textnormal{offspring} 1}}
\newcommand{\rchildb}{r_{\textnormal{offspring} 2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% optimal supply networks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\rhofac}{\rho_{\textnormal{fac}}}
\newcommand{\rhopop}{\rho_{\textnormal{pop}}}

%% supply networks

\newcommand{\volume}[1]{\Omega_{d,D}(#1)}

\newcommand{\vnet}{V_{\rm net}}

%% chaotic contagion

\newcommand{\niprob}{q}
\newcommand{\liprob}{r}


%% random biparite networks

\newcommand{\rbone}{\textnormal{\faFilm}}
\newcommand{\rbtwo}{\textnormal{\faLightbulbO}}

\newcommand{\rboneng}{N_{\rbone}}
\newcommand{\rbtwong}{N_{\rbtwo}}

\newcommand{\Prboneind}{P^{(\rbone)}_{\textnormal{ind},k}}
\newcommand{\Prbtwoind}{P^{(\rbtwo)}_{\textnormal{ind},k}}

\newcommand{\Rrboneind}{R^{(\rbone)}_{\textnormal{ind},k}}
\newcommand{\Rrbtwoind}{R^{(\rbtwo)}_{\textnormal{ind},k}}

\newcommand{\Prboneindplain}{P^{(\rbone)}_{\textnormal{ind}}}
\newcommand{\Prbtwoindplain}{P^{(\rbtwo)}_{\textnormal{ind}}}

\newcommand{\Rrboneindplain}{R^{(\rbone)}_{\textnormal{ind}}}
\newcommand{\Rrbtwoindplain}{R^{(\rbtwo)}_{\textnormal{ind}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% happiness

\newcommand{\havg}[1]{h_{\rm avg}(#1)}
\newcommand{\havgword}[1]{h_{\rm avg}(\textnormal{`#1'})}
\newcommand{\havgsup}[1]{h_{\rm avg}^{#1}}
\newcommand{\havgsuparg}[2]{h_{\rm avg}^{#1}(#2)}

\newcommand{\havgfn}{h_{\rm avg}}
\newcommand{\hstdfn}{h_{\textnormal{std}}}

\newcommand{\havgfnamb}{h_{\rm avg}^{\rm (amb)}}
\newcommand{\havgfnnorm}{h_{\rm avg}^{\rm (norm)}}


\newcommand{\Tref}{T_{\textnormal{ref}}}
\newcommand{\Tcomp}{T_{\textnormal{comp}}}

\newcommand{\deltahw}{\delta_{h}(w)}
\newcommand{\deltapw}{\delta_{p}(w)}



%% contagion
\newcommand{\vuln}{\textnormal{vuln}}
\newcommand{\trig}{\textnormal{trig}}
\newcommand{\Svuln}{S_{\textnormal{vuln}}}
\newcommand{\thetavuln}{\theta_{\textnormal{vuln}}}
\newcommand{\Strig}{S_{\textnormal{trig}}}
\newcommand{\Ptrig}{P_{\textnormal{trig}}}
\newcommand{\Sgc}{S_{\textnormal{gc}}}

\newcommand{\emn}{e_{\mu\nu}}
\newcommand{\emm}{e_{\mu\mu}}
\newcommand{\exx}{e_{x y}}
\newcommand{\exy}{e_{x x}}
\newcommand{\ejk}{e_{j k}}
\newcommand{\ejj}{e_{j j}}
\newcommand{\ekj}{e_{k j}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 80/20 rule, Gini coefficient
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\fracsymbol}{\theta}
\newcommand{\popfrac}{\fracsymbol_{\textnormal{pop}}}
\newcommand{\wealthfrac}{\fracsymbol_{\textnormal{wealth}}}
\newcommand{\ginicoefficient}{G}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Zipf, Simon's scaling
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% simon's model
\newcommand{\simonalpha}{\rho}

\newcommand{\simonrho}{\rho}
%% \newcommand{\zipfrank}{r}
%% \newcommand{\zipfexponent}{\alpha}
%% \newcommand{\frequency}{f}
\newcommand{\probsymbol}{p}
\newcommand{\zipfrankmax}{\zipfrank_{\textnormal{max}}}


%% rank for Zipf's law
\newcommand{\rank}{r}

%% rich gets richer model

%% same as simonrho

\newcommand{\zipfrank}{r}
\newcommand{\zipfexponent}{\alpha}

\newcommand{\groupnum}{n}

\newcommand{\innovationrate}{\rho}
\newcommand{\innovationratet}{\rho_{t}}

\newcommand{\rgrN}{S}
\newcommand{\Ngroups}{N}

%% \newcommand{\rgrNt}[1]{\rgrN_{#1}^{\textnormal{(e)}}}
%% \newcommand{\rgrNinit}{\rgrN^{\textnormal{(e,\textnormal{init})}}}
\newcommand{\rgrNt}[1]{\rgrN_{#1}}
\newcommand{\rgrNinit}{\rgrN^{\textnormal{\textnormal{init}}}}

\newcommand{\grouptimestart}[1]{t_{#1}^{\textnormal{init}}}

\newcommand{\groupsizet}[2]{\rgrN_{#1,#2}}
%% \newcommand{\groupsizet}[2]{\rgrN_{#1,#2}^{\textnormal{(e)}}}
%% \newcommand{\groupsizet}[2]{\rgrN_{#1}^{\textnormal{(e)}}(#2)}

\newcommand{\groupnumt}[1]{\Ngroups^{\textnormal{(g)}}_{#1}}

\newcommand{\rgrP}{P}
\newcommand{\groupprobt}[2]{\rgrP_{#1,#2}}
%% \newcommand{\groupprobt}[2]{\rgrP_{#1,#2}^{\textnormal{(e)}}}

\newcommand{\Beta}{B}

\newcommand{\onehalf}{\frac{1}{2}}
\newcommand{\onequarter}{\frac{1}{4}}


%% \newcommand{\Ngroupsinit}{\Ngroups_{\textnormal{init}}}
\newcommand{\groupnuminit}{\groupnum^{\textnormal{init}}}

%% language, lexical turbulence

%% language, zipf
\newcommand{\frequency}{f}

\newcommand{\frequencythreshold}{f_{\textnormal{thr}}}
%% \newcommand{\frequencythreshold}{f_{\Asterisk}}

\newcommand{\frequencyword}{f_{w;y}}
\newcommand{\frequencymedian}[2]{f_{w;#1,#2}^{\textnormal{med}}}
\newcommand{\frequencycut}[2]{f_{w;#1,#2}^{\textnormal{cut}}}


\newcommand{\flux}{\phi}
\newcommand{\fluxup}{\flux_{\textnormal{up}}}
\newcommand{\fluxdown}{\flux_{\textnormal{down}}}

\newcommand{\zipfexponentlower}{\alpha}
\newcommand{\zipfexponentupper}{\alpha'}

\newcommand{\fluxexponentlower}{\mu}
\newcommand{\fluxexponentupper}{\mu'}

\newcommand{\fluxrankexponentlower}{\nu}
\newcommand{\fluxrankexponentupper}{\nu'}

\newcommand{\breakpoint}{\textnormal{b}}
\newcommand{\zipfbreakpoint}{\zipfrank_{\breakpoint}}
%% \newcommand{\frequencythresholdbreakpoint}{{\frequencythreshold}_{,\textnormal{b}}}
\newcommand{\frequencythresholdbreakpoint}{f_{\breakpoint}}
 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% allotaxonometry:
%% 
%% universal categorical data shifts
%% 
%% - general 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\sizesymbol}{s}
\newcommand{\numbersymbol}{N}
\newcommand{\bigprobsymbol}{P}
\newcommand{\bigrank}{R}

\newcommand{\indexaraw}{1}
\newcommand{\indexbraw}{2}

\newcommand{\indexa}{(\indexaraw)}
\newcommand{\indexb}{(\indexbraw)}
\newcommand{\indexavg}{(\indexaraw\cdot\indexbraw)}

\newcommand{\indexref}{\textnormal{(ref)}}

\newcommand{\indexanyraw}{i}
\newcommand{\indexany}{(\indexanyraw)}

\newcommand{\measuresymbol}{\phi}
\newcommand{\bigmeasuresymbol}{\Phi}


\newcommand{\systemsymbol}{\Omega}
\newcommand{\elementsymbol}{\tau}

\newcommand{\elementsetsymbol}{\mathcal{T}}
\newcommand{\elementsetsymbola}{\mathcal{T}^{\indexa}}
\newcommand{\elementsetsymbolb}{\mathcal{T}^{\indexb}}
\newcommand{\elementsetsymbolany}{\mathcal{T}^{\indexany}}

\newcommand{\systema}{\systemsymbol^{\indexa}}
\newcommand{\systemb}{\systemsymbol^{\indexb}}
\newcommand{\systemavg}{\systemsymbol^{\indexavg}}
\newcommand{\systemref}{\systemsymbol^{\indexref}}
\newcommand{\systemany}{\systemsymbol^{\indexany}}

\newcommand{\Ntypesa}{\numbersymbol_{\indexaraw}}
\newcommand{\Ntypesb}{\numbersymbol_{\indexbraw}}
%% \newcommand{\Ntypesa}{\numbersymbol_{\systema}}
%% \newcommand{\Ntypesb}{\numbersymbol_{\systemb}}

\newcommand{\sizea}{\sizesymbol^{\indexa}}
\newcommand{\sizeb}{\sizesymbol^{\indexb}}
\newcommand{\sizeany}{\sizesymbol^{\indexany}}

\newcommand{\texta}{\textsymbol^{\indexa}}
\newcommand{\textb}{\textsymbol^{\indexb}}
\newcommand{\textany}{\textsymbol^{\indexany}}

\newcommand{\numbera}{\numbersymbol^{\indexa}}
\newcommand{\numberb}{\numbersymbol^{\indexb}}
\newcommand{\numberany}{\numbersymbol^{\indexany}}

\newcommand{\proba}{\probsymbol^{\indexa}}
\newcommand{\probb}{\probsymbol^{\indexb}}
\newcommand{\probavg}{\probsymbol^{\indexavg}}
\newcommand{\probany}{\probsymbol^{\indexany}}

\newcommand{\probmixedab}{\probsymbol^{(\indexaraw,\indexbraw)}}

\newcommand{\measurea}{\measuresymbol^{\indexa}}
\newcommand{\measureb}{\measuresymbol^{\indexb}}
\newcommand{\measureavg}{\measuresymbol^{\indexavg}}
\newcommand{\measureany}{\measuresymbol^{\indexany}}
\newcommand{\measureref}{\bigmeasuresymbol_{\systemref}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Entropy, Divergences
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\diffsummand}{\delta\bigmeasuresymbol_{\elementsymbol}(\systemb,\systema)}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% rank divergence
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\rtd}[1]{D^{\textnormal{R}}_{#1}}
\newcommand{\rtdelement}[1]{\delta D^{\textnormal{R}}_{#1,\elementsymbol}}

\newcommand{\rtdhalf}{\rtd{\sfrac{1}{2}}}
\newcommand{\rtdhalfelement}{\rtdelement{\sfrac{1}{2}}}

\newcommand{\rtdalpha}{\rtd{\alpha}}
\newcommand{\rtdalphaelement}{\rtdelement{\alpha}}

%% alpha as a variable
\newcommand{\rtdalphavar}[1]{\rtd{#1}}
\newcommand{\rtdalphavarelement}[1]{\rtdelement{#1}}

%% \newcommand{\rtdnorm}{C_{\textnormal{\bigrank}}}
%% \newcommand{\rtdnorm}{\mathcal{N}_{\textnormal{\bigrank}}}
%% \newcommand{\rtdnorm}{\mathcal{N}_{\bigrank_{\indexaraw,\indexbraw;\alpha}}}
\newcommand{\rtdnorm}{\mathcal{N}_{\indexaraw,\indexbraw;\alpha}}
\newcommand{\invrtdnorm}{\frac{1}{\rtdnorm}}

\newcommand{\rtdnormalpha}[1]{\mathcal{N}_{\indexaraw,\indexbraw;#1}}
\newcommand{\invrtdnormalpha}[1]{\frac{1}{\rtdnormalpha{#1}}}

\newcommand{\rtdalphasystems}[2]{\rtdalpha(#1\,\|\,#2)}
\newcommand{\rtdalphasystemsOmega}{\rtdalphasystems{\systemsymbol_{\indexaraw}}{\systemsymbol_{\indexbraw}}}
\newcommand{\rtdalphasystemsRank}{\rtdalphasystems{\bigrank_{\indexaraw}}{\bigrank_{\indexbraw}}}
\newcommand{\rtdalphasystemsRankRand}{\rtdalphasystems{\bigrank_{\indexaraw}}{\bigrank_{\indexbraw}}}

\newcommand{\rtdalphavarsystems}[3]{\rtdalphavar{#1}(#2\,\|\,#3)}
\newcommand{\rtdalphavarsystemsOmega}[1]{\rtdalphavarsystems{#1}{\systemsymbol_{\indexaraw}}{\systemsymbol_{\indexbraw}}}
\newcommand{\rtdalphavarsystemsRank}[1]{\rtdalphavarsystems{#1}{\bigrank_{\indexaraw}}{\bigrank_{\indexbraw}}}

\newcommand{\rtdalphavarsystemsRankRand}[1]{\rtdalphavarsystems{#1; \textnormal{rand}}
   {\bigrank_{\indexaraw}}
   {\bigrank_{\indexbraw}}}

%% \newcommand{\rtdalphavarsystemsRankRand}[1]{D^{\textnormal{R,rand}}_{#1}
%%  (\bigrank_{\indexaraw}\,\|\,\bigrank_{\indexbraw})}

%% merged systems, ordering of contributions for rank probability
\newcommand{\bigrankordering}{\bigrank_{\indexaraw,\indexbraw;\alpha}}
\newcommand{\bigrankorderingalpha}[1]{\bigrank_{\indexaraw,\indexbraw;#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% probability divergence
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\probdiv}[1]{D^{\textnormal{P}}_{#1}}
\newcommand{\probdivelement}[1]{D^{\textnormal{P}}_{#1,\elementsymbol}}

\newcommand{\probdivhalf}{\probdiv{\sfrac{1}{2}}}
\newcommand{\probdivhalfelement}{\probdivelement{\sfrac{1}{2}}}

\newcommand{\probdivalpha}{\probdiv{\alpha}}
\newcommand{\probdivalphaelement}{\probdivelement{\alpha}}

%% normalization factor

\newcommand{\ptdnorm}{\mathcal{N}_{\indexaraw,\indexbraw;\alpha}^{\textnormal{P}}}
\newcommand{\invptdnorm}{\frac{1}{\ptdnorm}}

\newcommand{\ptdnormalpha}[1]{\mathcal{N}_{\indexaraw,\indexbraw;#1}^{\textnormal{P}}}
\newcommand{\invptdnormalpha}[1]{\frac{1}{\ptdnormalpha{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% generalized entropy divergence
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\gendiv}[1]{D^{\textnormal{AS2}}_{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% jensen-shannon divergence
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\jsd}{D^{\textnormal{JS}}}
\newcommand{\kld}{D^{\textnormal{KL}}}

\newcommand{\jsdelement}{D^{\textnormal{JS},\elementsymbol}}
\newcommand{\kldelement}{D^{\textnormal{KL},\elementsymbol}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% universal categorical data shifts
%% texts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\textsymbol}{T}

\newcommand{\logtwo}{\textnormal{log}_2}



